CO or no CO? Narrowing the CO abundance constraint and recovering the H2O detection in the atmosphere of WASP-127 b using SPIRou

Precise measurements of chemical abundances in planetary atmospheres are necessary to constrain the formation histories of exoplanets. A recent study of WASP-127b, a close-in puffy sub-Saturn orbiting its solar-type host star in 4.2 d, using HST and Spitzer revealed a feature-rich transmission spectrum with strong excess absorption at 4.5 um. However, the limited spectral resolution and coverage of these instruments could not distinguish between CO and/or CO2 absorption causing this signal, with both low and high C/O ratio scenarios being possible. Here we present near-infrared (0.9--2.5 um) transit observations of WASP-127 b using the high-resolution SPIRou spectrograph, with the goal to disentangle CO from CO2 through the 2.3 um CO band. With SPIRou, we detect H2O at a t-test significance of 5.3 sigma and observe a tentative (3 sigma) signal consistent with OH absorption. From a joint SPIRou + HST + Spitzer retrieval analysis, we rule out a CO-rich scenario by placing an upper limit on the CO abundance of log10[CO]<-4.0, and estimate a log10[CO2] of -3.7^(+0.8)_(-0.6), which is the level needed to match the excess absorption seen at 4.5um. We also set abundance constraints on other major C-, O-, and N-bearing molecules, with our results favoring low C/O (0.10^(+0.10)_(-0.06)), disequilibrium chemistry scenarios. We further discuss the implications of our results in the context of planet formation. Additional observations at high and low-resolution will be needed to confirm these results and better our understanding of this unusual world.

==> tab_params_mcmc_wasp.tex <==
%\onecolumngrid
% \LongTables
% \tabletypesize{\normalsize}
\begin{table*}
% \tablewidth{0pt}
% \tablecolumns{6}
\caption{MCMC Retrieval Parameter Priors and Results \label{tab:param_MCMC_a2}}
\begin{threeparttable}
\begin{tabular}{lcrrrc}
\hline
Parameter  & Priors & SPIRou only & HST+Spitzer only  & SPIRou+HST+Spitzer  & Unit \\
\hline
% --- planet parameters
$\log_{10}$ \water & $\mathcal{U}(-12,-0.1)$              & $-2.71_{-0.56}^{+0.64}$  &  $-1.84_{-0.42}^{+0.70}$  &  $-3.27_{-0.57}^{+0.46}$ &  \\ 
$\log_{10}$ CO & $\mathcal{U}(-12,-0.1)$                  & $< -3.98$  &  $< -1.39$  &  $< -4.23$ &  \\ 
$\log_{10}$ \diox & $\mathcal{U}(-12,-0.1)$               & $-7.43_{-1.90}^{+4.29}$  &  $-3.09_{-0.58}^{+0.82}$  &  $-4.00_{-0.77}^{+0.64}$ &  \\ 
$\log_{10}$ FeH & $\mathcal{U}(-12,-0.1)$                 & $< -8.68$  &  $< -4.10$  &  $< -9.00$ &  \\ 
$\log_{10}$ \methane & $\mathcal{U}(-12,-0.1)$            & $< -4.33$  &  $< -5.07$  &  $< -6.49$ &  \\ 
$\log_{10}$ HCN & $\mathcal{U}(-12,-0.1)$                 & $< -4.54$  &  $< -4.28$  &  $< -5.27$ &  \\ 
$\log_{10}$ NH$_3$ & $\mathcal{U}(-12,-0.1)$              & $< -5.31$  &  $< -4.36$  &  $< -5.97$ &  \\ 
$\log_{10}$ C$_2$H$_2$ & $\mathcal{U}(-12,-0.1)$          & $< -5.79$  &  $< -4.50$  &  $< -6.40$ &  \\ 
$\log_{10}$ TiO & $\mathcal{U}(-12,-0.1)$                 & $< -3.59$  &  $< -7.26$  &  $< -8.88$ &  \\ 
$\log_{10}$ OH & $\mathcal{U}(-12,-0.1)$                  & $-2.48_{-0.54}^{+0.67}$  &  $-5.94_{-2.86}^{+3.76}$  &  $-2.97_{-0.72}^{+0.86}$ &  \\ 
$\log_{10}$ Na & $\mathcal{U}(-12,-0.1)$                  & $\cdots$  &  $-4.96_{-2.33}^{+3.58}$  &  $-6.88_{-1.98}^{+2.17}$ &  \\ 
$\log_{10}$ K & $\mathcal{U}(-12,-0.1)$                   & $\cdots$  &  $< -2.83$  &  $< -5.91$ &  \\ 
$T_{\rm P}$ & $\mathcal{U}(400, 2000)$                    & $865_{-183}^{+213}$  &  $1220_{-220}^{+268}$  &  $862_{-116}^{+180}$ & K \\ 
$\log_{10} P_{\rm cloud}$ & $\mathcal{U}(-6.0, 0.0)$      & $> -3.42$  &  $> -3.64$  &  $> -2.63$ & bar \\ 
$R_{\rm P}$ & $\mathcal{U}(1.0, 1.6)$                     & $1.28_{-0.02}^{+0.03}$  &  $1.22_{-0.04}^{+0.03}$  &  $1.29_{-0.01}^{+0.02}$ & $R_J$ \\ 
$\gamma$ & $\mathcal{U}(-6.0, 0.0)$                       & $\cdots$  &  $-1.81_{-0.74}^{+0.93}$  &  $-1.80_{-0.77}^{+0.90}$ &  \\ 
$\log_{10} S$ & $\mathcal{U}(-10.0, 4.0)$                 & $\cdots$  &  $1.87_{-0.52}^{+0.75}$  &  $-0.04_{-0.69}^{+0.85}$ &  \\ 
$K_{\rm P}$ & $\mathcal{G}(129.95, 1.2)$                  & $130.34_{-1.25}^{+1.11}$  &  $\cdots$  &  $130.06_{-1.25}^{+1.14}$ & km s$^{-1}$ \\ 
$v_{\rm rad}$ & $\mathcal{U}(-10.0, 10.0)$                & $-0.14_{-0.53}^{+0.65}$  &  $\cdots$  &  $-0.20_{-0.67}^{+0.66}$ & km s$^{-1}$ \\ 
$\omega$ & $\mathcal{U}(0, 15)$                           & $9.35_{-0.52}^{+0.44}$  &  $\cdots$  &  $9.26_{-0.41}^{+0.49}$ & d$^{-1}$ \\ 
$f_{\rm R}$ & $\mathcal{U}(0, 1.0)$                       & $0.44_{-0.09}^{+0.10}$  &  $\cdots$  &  $0.39_{-0.09}^{+0.08}$ &  \\ 
% --- orbital params
% ---- Abundance ratios
\hline
 C/O  & $\cdots$                                          & $0.02_{-0.02}^{+0.01}$  &  $0.04_{-0.03}^{+0.07}$  &  $0.04_{-0.03}^{+0.04}$ &  \\ 
$[$C/H$]^a$ & $\cdots$                                    & $-1.42_{-1.36}^{+1.28}$  &  $0.50_{-0.85}^{+0.64}$  &  $-0.68_{-0.69}^{+0.69}$ &  \\ 
$[$O/H$]^a$ & $\cdots$                                    & $0.94_{-0.45}^{+0.55}$  &  $1.45_{-0.40}^{+0.59}$  &  $0.41_{-0.63}^{+0.64}$ &  \\ 
\hline
 C/O  & $\cdots$                                          & $0.02_{-0.02}^{+0.01}$  &  $0.04_{-0.03}^{+0.08}$  &  $0.10_{-0.06}^{+0.10}$ &  No OH \\ 
$[$C/H$]^a$ & $\cdots$                                    & $-0.55_{-1.87}^{+0.94}$  &  $0.51_{-0.86}^{+0.64}$  &  $-0.23_{-0.68}^{+0.66}$ &  No OH \\  
$[$O/H$]^a$ & $\cdots$                                    & $0.84_{-0.64}^{+0.61}$  &  $1.40_{-0.43}^{+0.62}$  &  $0.22_{-0.60}^{+0.57}$ &  No OH \\ 
% C/H$_{*}$ & $\cdots$   & $-1.21_{-0.56}^{+0.61}$  &  $-0.22_{-1.03}^{+0.89}$  &  $-1.22_{-0.41}^{+0.38}$ &  \\
% O/H$_{*}$ & $\cdots$  & $0.31_{-0.58}^{+0.66}$  &  $0.46_{-0.67}^{+0.56}$  &  $-0.17_{-0.47}^{+0.34}$ &  \\
% N/H (solar) & $\cdots$  & $1.6\inc{}{}$ & $5.5\inc{}{}$ & $0.3\inc{}{}$ &   
% N/H & \cdots  & $0.01\inc{}{}$ & $0.10\inc{}{}$ & $0.9\inc{}{}$ &   \\
\hline
\end{tabular}

\begin{tablenotes}
\item \textsc{\textbf{Notes}} --- The marginalized parameters from the likelihood analysis with their $\pm 1\,\sigma$ errors, or their 2$\sigma$ upper or lower limits. The log of the VMR are unitless. $^a$Abundances ratios compared to the solar value in $\log_{10}$.
\end{tablenotes}
\end{threeparttable}
\end{table*}


